MegaFace: A Million Faces for Recognition at Scale

Recent face recognition experiments on the LFW benchmark show that face recognition is performing stunningly well, surpassing human recognition rates. In this paper, we study face recognition at scale. Specifically, we have collected from Flickr a \textbf{Million} faces and evaluated state of the art face recognition algorithms on this dataset. We found that the performance of algorithms varies--while all perform great on LFW, once evaluated at scale recognition rates drop drastically for most algorithms. Interestingly, deep learning based approach by \cite{schroff2015facenet} performs much better, but still gets less robust at scale. We consider both verification and identification problems, and evaluate how pose affects recognition at scale. Moreover, we ran an extensive human study on Mechanical Turk to evaluate human recognition at scale, and report results. All the photos are creative commons photos and is released at \small{\url{http://megaface.cs.washington.edu/}} for research and further experiments.

==> text/Recognition_Methods.tex <==


\section{Recognition Methods}

We have selected to experiment with four recognition algorithms that represent very different types of techniques. 

\paragraph{Basic LBP comparison.} We have implemented a  comparison based on Local Binary Pattern (LBP) descriptors.   \red{give details about what were the sizes, cell size, how many, chi square distance, ...}.  This approach achieves \red{xxx} recognition rates on LFW, and uses no training. 


\paragraph{Joint Bayesian.}   The Joint Bayesian model represents each face as the sum of two Gaussian variables
$$x = \mu + \epsilon$$ where $\mu$ represents identity and $\epsilon$ represents inter-personal variation.  To determine whether two faces, $x_1$ and $x_2$ belong to the same identity, we calculate $P(x_1, x_2 | H_1)$ and $P(x_1, x_2 | H_2)$ where $H_1$ is the hypothesis that the two faces are the same and $H_2$ is the hypothesis that the two faces are different. These distributions can also be written as normal distributions, which allows for efficent inference via a log-likelihood test. \red{add detail, trained on CASIA... achieves on LFW...}



%
%We experimented with several algorithms that achieve state-of-the-art performance on the LFW benchmark including Joint Bayesian and the commercial algorithms VisionLabs and Google FaceNet.
%In addition, we report and show large-scale results for the vanilla LBP descriptor.
%Joint Bayesian ... TODO: Explain what the Joint Bayesian algorithm does




\paragraph{Commercial software by VisionLabs.} 
VisionLabs achieved \red{xxx} recognition rates on LFW, is trained on outside data \red{???}. 

%Although VisionLabs has not published their algorithm it can be inferred that it is based on SIFT Fisher vector encoding combined with metric learning.

\paragraph{Googel's FaceNet} Google FaceNet \cite{schroff2015facenet} is the most recent and highest performing of several Deep Learning algorithms applied to the LFW benchmark. 
Unlike DeepFace and DeepID the FaceNet which have a bottleneck layer and are optimized by minimizing cross-entropy, FaceNet learns an embedding such that the extracted features are directly comparable using the Euclidean distance.
 It is  trained on 290 Million photos of 1.8 Million people. 
 

==> text/method.tex <==
\section{Evaluation Methodology}


